Barrier Certificate based Safe Control for LiDAR-based Systems under Sensor Faults and Attacks

Autonomous Cyber-Physical Systems (CPS) fuse proprioceptive sensors such as GPS and exteroceptive sensors including Light Detection and Ranging (LiDAR) and cameras for state estimation and environmental observation. It has been shown that both types of sensors can be compromised by malicious attacks, leading to unacceptable safety violations. We study the problem of safety-critical control of a LiDAR-based system under sensor faults and attacks. We propose a framework consisting of fault tolerant estimation and fault tolerant control. The former reconstructs a LiDAR scan with state estimations, and excludes the possible faulty estimations that are not aligned with LiDAR measurements. We also verify the correctness of LiDAR scans by comparing them with the reconstructed ones and removing the possibly compromised sector in the scan. Fault tolerant control computes a control signal with the remaining estimations at each time step. We prove that the synthesized control input guarantees system safety using control barrier certificates. We validate our proposed framework using a UAV delivery system in an urban environment. We show that our proposed approach guarantees safety for the UAV whereas a baseline fails.

==> framework_bc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Control Barrier Certificates}\label{sec:CBC}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we propose a framework based on control barrier certificates to ensure end-to-end safety. 

% \subsection{Control Barrier Certificates}
% \label{subsec:CBC}
We denote each estimation from sensor as $\hat{x}_i$ of sensor $i$. We denote the correct state estimation as $\hat{x}_{\alpha}[k]$

We define $\hat{u}$ and construct 
\begin{equation}
    x[k+1] = f(x[k]) + g(x[k]) (u[k]+\hat{u}[k]) + w[k]\xi[k]
\end{equation}
We can have 
\begin{equation}
    \begin{aligned}
        x_{k+1} = &f(x_k) + g(x_k) u(\hat{x}_{\alpha}[k]) + g(x_k) \hat{u}[k]  + w[k]\xi[k] \\
        \hat{x}_{k+1} =& f(\hat{x}_k) + g(x_k) u(\hat{x}_{\alpha}[k])  + K_k(o(x[k]) + v[k]\eta[k] - o(\hat{x}[k])) \\
        K_k =& A_{k} P_{k} C_{k}^{T}(C_{k} P_{k} C_{k}^{T}+R_{k})^{-1} \\
        P_{k+1} =& A_{k} P_{k} A_{k}^{T}+Q_{k}-K_{k}(C_{k} P_{k} C_{k}^{T}+R_{k}) K_{k}^{T}.
    \end{aligned}
\end{equation}
where $A_{k} =\frac{\partial f}{\partial x}(\hat{x}_{k}, u_{k}) $, $C_{k} =\frac{\partial h}{\partial x}(\hat{x}_{k})$

% and $P_k$ is defined by the Riccati difference equation
% \begin{equation*}
%     P_{k+1}=A_{k} P_{k} A_{k}^{T}+Q_{k}-K_{k}(C_{k} P_{k} C_{k}^{T}+R_{k}) K_{k}^{T}. 
% \end{equation*}

Define $\Bar{x}[k]=\left(x[k], \hat{x}_{\alpha}[k]\right)$ as an extended state vector, with
\begin{multline}
\label{eq:extend_dyn}
    \Bar{x}[k+1] = F(\Bar{x}[k], \hat{u}[k], w[k], v[k]) := f(\Bar{x}[k]) \\ + g(\Bar{x}[k]) (u(\bar{B} \hat{x}_{\alpha})+\hat{u}[k]) + \bar{W}_{k} w[k]\xi[k] + \bar{V}_{k} v[k]\eta[k], 
\end{multline}
where 
\begin{equation}
    \bar{B}_{k}=\left(\begin{array}{c}0 \\ I\end{array}\right), \quad
    \bar{W}_{k}=\left(\begin{array}{c}I \\ 0\end{array}\right), \quad \bar{V}_{k}=\left(\begin{array}{c}0 \\ K_k\end{array}\right). 
\end{equation}
% where $\hat{u}(t)$ satisfies $\|\hat{u}(t)\|_{2} \leq \xi$. 
In order to guarantee safety under any false data injection strategy of the adversary, we assume that $\hat{\mathbf{u}}(t)$ is a disturbance that $\hat{u}(t)$ satisfies $\|\hat{u}(t)\|_{2} \leq \xi$.


% \begin{equation}
%     \Bar{x}[k+1] = \left(\begin{array}{cc}A & B K \\ \Phi C_{\alpha}^{T} \Sigma_{v_{\alpha}} C_{\alpha} & A-\Theta C_{\alpha}+B K\end{array}\right)\left(\begin{array}{c}\mathbf{x}(t) \\ \hat{\mathbf{x}}_{\alpha}(t)\end{array}\right)
% \end{equation}

% where \textcolor{blue}{(Need to derive $f$ and $g$)}
% In order to guarantee safety under any false data injection strategy of the adversary, we assume that $\hat{\mathbf{u}}(t)$ is a disturbance that can take arbitrary values. Using the definition of $\mathbf{u}_{\alpha}(t)$, we can write an extended system as

% where $\Theta(t)= \Phi(t) C_{\alpha}^{T} \Sigma_{\mathbf{v}_{\alpha}}^{-1}$ and $ K(t)=-R^{-1} B^{T} P(t)$
% where \textcolor{blue}{(Need to derive $f$ and $g$)}
% \begin{equation}
%     \label{eq:extend_dyn}
%     % \Bar{x}[k+1] = [A_{k}]
% \end{equation}
% and 

% \begin{equation}
%     \bar{F}_{k}=\left(\begin{array}{c}w[k] \\ 0\end{array}\right), \quad \bar{G}_{k}=\left(\begin{array}{c}0 \\ v[k]\end{array}\right)
% \end{equation}

% $A_{k} =\frac{\partial f}{\partial x}(\hat{x}_{k}, u_{k}) $, $C_{k} =\frac{\partial h}{\partial x}(\hat{x}_{k})$

% \textcolor{blue}{(Use $\bar{x}$ to replace $x$ in Proposition 1 and 2)}
\begin{proposition}
\label{prop:discrete_bc}
    Consider a discrete-time system described by \eqref{eq:dynamic} and sets $\mathcal{C}, \mathcal{D} \subseteq \mathcal{X}$. If there exist a function $B: \mathcal{X} \rightarrow \mathbb{R}_{0}^{+}$as defined in Definition \ref{def:dt_BC} with constant $c \geq 0$, stationary policy $u: X \rightarrow U$ with $\|\hat{u}\|\leq \xi$, and a constant $\gamma \in[0,1)$ such that
    \begin{eqnarray}
        B(\bar{x}) \leq \gamma, & \  \forall \bar{x} \in \mathcal{C} \label{eq:prop1_1} \\
        B(\bar{x}) \geq 1, & \  \forall \bar{x} \in \mathcal{D} \label{eq:prop1_2}\\
        \mathbb{E}[B(F(\Bar{x}, \hat{u}, w, v)) \mid \bar{x}] \leq B(\bar{x})+c, & \ \forall \bar{x} \in \mathcal{X} \label{eq:prop1_3}
    \end{eqnarray}
    then for any constant $\lambda>0$ and any initial state $x_{0} \in \mathcal{X}$, we have the $Pr(x(k)\in C, 0\leq k\leq T_d)\geq 1-\gamma- c T_d$. 
    % \begin{multline}
    %     Pr \left\{x(k) \in \mathcal{D}\right.\text{for some }\left.0 \leq k<T_{d} \mid x(0)=x_{0}\right\} \\
    %     \leq P\left\{\sup _{0 \leq k<T_{d}} B(x(k)) \geq 1 \mid x(0)=x_{0}\right\} \\
    %     \leq B\left(x_{0}\right)+c T_{d} \leq\gamma+c T_{d}. 
    % \end{multline}
\end{proposition}
% \begin{proposition}
% \label{prop:discrete_bc}
%     Consider a discrete-time system described by \eqref{eq:dynamic} and sets $\mathcal{C}, \mathcal{D} \subseteq \mathcal{X}$. If there exist a function $B: \mathcal{X} \rightarrow \mathbb{R}_{0}^{+}$as defined in Definition \ref{def:dt_BC} with constant $c \geq 0$, stationary policy $u: X \rightarrow U$ with $\|u\|\leq \xi$, and a constant $\gamma \in[0,1)$ such that
%     \begin{eqnarray}
%         B(\bar{x}) \leq \gamma, & \  \forall \bar{x} \in \mathcal{C} \label{eq:prop1_1} \\
%         B(\bar{x}) \geq 1, & \  \forall \bar{x} \in \mathcal{D} \label{eq:prop1_2}\\
%         \min_{u \in U} \mathbb{E}[B(F(\Bar{x}[k], \hat{u}[k], w[k], v[k])) \mid \bar{x}, u] \leq B(\bar{x})+c, & \ \forall \bar{x} \in \mathcal{X} \label{eq:prop1_3}
%     \end{eqnarray}
%     then for any constant $\lambda>0$ and any initial state $x_{0} \in \mathcal{X}$, we have the $Pr(x(k)\in C, 0\leq k\leq T_d)\geq 1-\gamma- c T_d$. 
%     % \begin{multline}
%     %     Pr \left\{x(k) \in \mathcal{D}\right.\text{for some }\left.0 \leq k<T_{d} \mid x(0)=x_{0}\right\} \\
%     %     \leq P\left\{\sup _{0 \leq k<T_{d}} B(x(k)) \geq 1 \mid x(0)=x_{0}\right\} \\
%     %     \leq B\left(x_{0}\right)+c T_{d} \leq\gamma+c T_{d}. 
%     % \end{multline}
% \end{proposition}

\begin{proof}
    The proof combines Lemma 3.5 and Theorem 3.6 in \cite{jagtap2020formal}. 
    Since there exists a function $B(x)$ satisfy \eqref{eq:prop1_3}, $B(x)$ is a Control Barrier Certificate for discrete-time system \eqref{eq:dynamic}. According to Lemma 3.5 and \eqref{eq:prop1_2}, we can have
    \begin{multline}
        Pr \left\{x(k) \in \mathcal{D}\right.\text{for some }\left.0 \leq k<T_{d} \mid x(0)=x_{0}\right\} \\
        \leq P\left\{\sup _{0 \leq k<T_{d}} B(x(k)) \geq 1 \mid x(0)=x_{0}\right\} \\
        \leq B\left(x_{0}\right)+c T_{d} \leq\gamma+c T_{d}. 
    \end{multline}
\end{proof}

The system has continuous state space $\mathcal{X}$ and action space $U$, we can follow the standard procedure to compute control barrier certificate $B(x)$ by solving an SOS programming. We define 
\begin{equation}
    h_{B}^{\xi}(u_i)=\xi^{2}-\sum_{i=1}^{m} u_{i}^{2}
\end{equation}

\begin{proposition}
Suppose there exists a function $B(\bar{x})$ and polynomials $\lambda_0(\bar{x})$, $\lambda_1(\bar{x})$, $\lambda_x(\bar{x},u)$ and $\lambda_u(\bar{x},u)$ such that
\begin{eqnarray}
    -B(\bar{x})-\lambda_{0}^{T}(\bar{x}) h_{0}(\bar{x})+\gamma & \geq & 0 \label{eq:prop2_1}\\
    B(\bar{x})-\lambda_{1}^{T}(\bar{x}) h_{1}(\bar{x})-1 & \geq & 0  \label{eq:prop2_2}\\
    -\mathbb{E}[B(F(\Bar{x}, \hat{u}, w, v)) \mid \bar{x}]+B(\bar{x}) \nonumber \\
    -\lambda_{u}^{T}(\bar{x}, u) h_{B}^{\xi}(u) +c & \geq & 0. \label{eq:prop2_3}
\end{eqnarray}
Then $B(x)$ satisfy the condition in Proposition \ref{prop:discrete_bc} and any $u\in \{u:\|u\| \leq \xi \}$ is the corresponding control input.
\end{proposition}
% -\lambda_{\bar{x}}^{T}(\bar{x}, u) h(\bar{x})+c

\begin{proof}
Since the entries $B(x)$ and $\lambda_{0}(x)$ in $-B(x)-\lambda_{0}^{T}(x) h_{0}(x)+\gamma$ are SOS, we have $0 \leq B(x)+\lambda_{0}^{T}(x) h_{0}(x) \leq \gamma$. Since the term $\lambda_{0}^{T}(x) h_{0}(x)$ is nonnegative over $\mathcal{C}$, \eqref{eq:prop2_1} and \eqref{eq:prop2_2} implies \eqref{eq:prop1_1} and \eqref{eq:prop1_2} in Proposition \ref{prop:discrete_bc}. 
Since the terms $\lambda_{u}^{T}(x, u) h_{B}^{\xi}(u)$ and $\lambda_{x}^{T}(x) g(x)$ are nonnegative over set $\mathcal{X}$, we have $\mathbb{E}[B(f(x, u, w)) \mid x, u] \leq B(x)+c$, which implies that the function $B(x)$ is a control barrier certificate.
\end{proof}

The choice of $\xi$ refers to \cite{niu2019lqg} Section.III C. 


% \subsection{Control Barrier Certificate Synthesis}
% \label{subsec:CBC_syt}








% However, it can be challenging to determine which sensor is more trust-worthy than others. 

% We further consider the case where the system is under the threat of input perturbations during online phase. We propose a hybrid fault-tolerant framework to passively ensure safety and actively exclude sensors experiencing fault or perturbations.
% We suppose that the false data is injected with purposes to bias the estimations of states, environment or both at the same time. Hence, the defense strategy aims to remove the false estimation by dealing with the impact separately.



% We further grind our proposed method on a LiDAR-based system. 

\iffalse

In what follows, we illustrate the fault tolerant scheme in two-fold, that is fault tolerant state estimation and safety guarantee introduced in the next section. The basic idea of our approach is to utilize additional information contained in high-dimensional sensor measurements as is summarized in Fig. \ref{fig:FT-est}. 


\subsection{Fault Tolerant State Estimation}

We further consider the case where the system is under the threat of input perturbations during online phase. We propose a hybrid fault tolerant framework to passively ensure safety and actively exclude sensors experiencing fault or perturbations.
We suppose that the false data is injected with purposes to bias the estimations of states, environment or both at the same time. Hence, the defense strategy aims to remove the false estimation by dealing with the impact separately.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/FT-Estimation.png}
    \caption{Fault Tolerant State Estimation with HD Sensors}
    \label{fig:FT-est}
\end{figure}



% \subsection{Propose Fault Tolerant Control}

% Intuitively, Control Constraint based on \eqref{eq:bc_safe_con} to ensures safety under perturbations $u(\hat{x}\mid \mathcal{T},\Bar{\mathcal{I}})\in \mathcal{K}_{cbf}$. 

% Theorem 2 $Z[k]=\{y(x[k]), \mathcal{O}(\Bar{\mathcal{I}})\}$



We then select parameters for fault tolerance $\theta_l, \theta_h>0$ and $\delta>0$. The set of feasible control actions is defined at each time-step $k$ using the following steps:
\begin{enumerate}
    \item Define state estimation excluding sensor $i$ as $\hat{x}_{k,i}$ and control input $u_i:=\pi(\hat{x}_{k,i})$. Define a collection of a set $\Omega_{i\in I}:= (u-u_i)^T (u-u_i) \leq \eta$. 
    % \begin{multline}
    % \label{eq:safecons}
    %     \Omega_i \triangleq \{ -\mathbb{E}[B(f(\hat{x}_{k,i})+g(\hat{x}_{k,i})u[k]) \mid \hat{x}_{k,i}]+ \\ \frac{B(\hat{x}_{k,i})}{\tilde{\alpha}} 
    %     +\tilde{\beta} -\lambda_{\mathcal{X} \backslash \mathcal{X}_{u}}(x) s_{\mathcal{X} \backslash \mathcal{X}_{u}}(x) \in \Sigma[x]  \} 
    % \end{multline}
    If control input $u$ satisfies $u[k] \in \bigcap_{i\in I} \Omega_{i}$, set $u_{\alpha}[k]=0$. Otherwise, select $u_{\alpha}[k]$ such that $u_o:=u+u_{\alpha}$ is the solution to the following QCQP problem. \textcolor{blue}{(Working on notations and QCQP)}
    \begin{equation}
    \begin{split}
        \min_{u_o} \ &{u_o^{T} R u_o+\hat{x}_i[k]^{T} P[k] B u_o+s[k]^{T} B u_o}\\
        s.t. \ & u_o \in \bigcap_{i\in I} \Omega_{i}
    \end{split}
    \end{equation}
    If no such $u_{t}$ exists, then go to Step 2. 
    
    \item For each $i$ with $ScanMatch(\mathcal{O}_i(\hat{x}_{k,i}, \mathcal{M}), \mathcal{O}(x_k,\Bar{\mathcal{I}}))>\theta_{h}$, we consider the following two cases: \\
    \textbf{Case I: } If $i$ with $\left\|\hat{x}_{k, i}-\hat{x}_{k, I\backslash i}\right\|_{2}>\theta_{l}$, exclude sensor with index $i$ and set $\Omega_{k}=\Omega_{k} \backslash\{i\in I_l\}$. \\
    \textbf{Case II: } Otherwise, exclude observation $\mathcal{O}$ and set $\Omega_{k}=\Omega_{k} \backslash\{i \in I_h\}$. \\
    For the above cases, if $\bigcap_{i\in I} \Omega_{i} \neq \emptyset$, then select $u_{k} \in \bigcap_{i\in I} \Omega_{i}$. Else go to Step 3 .
    
    % For each $i, j$ with $\left\|\hat{x}_{t, i}-\hat{x}_{t, j}\right\|_{2}>\theta_{i j}$, set $Z_{t}=Z_{t} \backslash\{i\}$ (resp. $Z_{t}=Z_{t} \backslash\{j\}$ ) if $\left\|\hat{x}_{t, i}-\hat{x}_{t, i, j}\right\|_{2}>\theta_{i j} / 2$ (resp. $\left.\left\|\hat{x}_{t, j}-\hat{x}_{t, i, j}\right\|_{2}>\theta_{i j} / 2\right)$. If $\bigcap_{i \in Z_{t}} \Omega_{i} \neq \emptyset$, then select $u_{t} \in \bigcap_{i \in Z_{t}} \Omega_{i}$. Else go to Step 3 .
    
    \item Remove the indices $i$ from $Z_{t}$ corresponding to the estimators with the largest residue values $\bar{y}_{k, i}-\bar{h}_{i} (\hat{x}_{t, i})$ until there exists $u_{k} \in \bigcap_{i \in Z_{t}} \Omega_{i}$.
\end{enumerate}


% Algorithm (transformation) = ML-NDT$(R,S,q,n,s)$

% \begin{algorithm}
% \caption{Fault Tolerant Control}
% \begin{algorithmic}
%     \State Given a safe region $\mathcal{C}$ and an accurate map $\mathcal{M}$
%     \State Given a verified safe trajectory $\mathcal{T}_s$. 
%     \For{$k\leq K$}
%         \State Fault Tolerant State Estimation $\hat{x}[k]$ with index $I[k]$.
%         \State Choose $u\in \Omega_{I[k]}$
%     \EndFor
% \end{algorithmic}
% \label{alg:FTCon}
% \end{algorithm}

% To ensure the system remain in safe region under adversarial attack, we consider the worst-case scenario when conducting safety verification.  
% The control module $u(\hat{x}[k], \mathcal{T})$ maps state estimation $\hat{x}[k]$ with a given trajectory $\mathcal{T}$ to control input $u[k]$ to maneuver the physical plant. 

% \subsection{Performance Trade-off}
% \begin{proposition}
% Verified safe trajectories $\mathcal{T}_s\in \Bar{\mathcal{T}}$ generated by planner who ensures convergence inherit the property of convergence.  
% \end{proposition}

% \subsection{Compatibility}
% We illustrate how our approach 
% To improve the compatibility to some path planning algorithms that focus more on performance, we propose a 

% term hd sensor and ld sensor
% low-dim sensors can be expressed as $y=\pi(x)$ but high-dim sensors need to be processed with filters feature extraction and etc. 

% this section is not novel
% focus more on perturbations

\subsection{Fault Tolerant Control}
% \textcolor{blue}{This subsection is going to be split into two-fold: ft-estimator and ft-control. The ft-control comes from ft-estimator which allow us passively ensure safety and exclude the false sensors at the same time. }
% We first propose a fault-tolerant estimator that excludes false sensors

% (The adversary can attack any sensor or combination of sensors. We assume he system under attack is still uniformly observable. )
We assume he system under attack is still uniformly observable.
Let $I_a\subsetneq I_l$ be a set of indices of sensors and let the distance between estimation $i$ and $j$ be $\zeta_{i,j}:=\|\hat{x}_{i}-\hat{x}_j\|$. 
We further define the following cases as criteria to exclude false sensors. 
\begin{itemize}
    \item Case I: $I_a = \emptyset$, if for any sensors $i,j\in I_l$ ($i\neq j$), $\zeta_{i,j}\leq \theta_l$. 
    \item Case II: LiDAR sensors are secure, if for any LiDAR scan $z$, $\zeta_z^s \leq \bar{\zeta}^s$ % and $\tilde{\zeta_z}^s \leq \bar{\zeta}^s$. 
    \item Case III: $i \notin I_a$, if for sensor indexing $i\in I_l$ Case I does not hold but Case II holds with $\|r_i\|\leq \theta_h$. 
    \item Case IV: If for sensor indexing $i\in I_l$ Case I and II do not hold. We consider the following cases. 
    \begin{itemize}
        \item a) LiDAR scan $z$ is not secure but scan $\tilde{z}$ is secure if $\zeta_z^s \geq \bar{\zeta}^s$ and $\tilde{\zeta}_z^s \leq \bar{\zeta}_z^s$. 
        \item b) $i \notin I_a$ if $\|\tilde{r}_i\|\leq \theta_h^i$ and $\tilde{\zeta}_z^s \leq \bar{\zeta}^s$. Otherwise, the LiDAR scan and sensor $i$ are joint attacked by the adversary, which means $i \in I_a$. 
    \end{itemize}
\end{itemize}
We consider the sensors are secure if Case I holds. Otherwise, there at least exists one sensor experiencing fault. Similarly, we consider the LiDAR sensors are secure if Case II holds. Otherwise, there at least exists one laser measurement spoofed. 
If sensor $i$ is away from other estimations and exceeding the threshold $\theta_l$, it can be the case that either sensor $i$ is under attack or other sensors except $i$ are spoofed. 
We use LiDAR sensor to help identify the fault. If Case II hold $\|r_i\|\leq \theta_h$ for sensor $i$ in Case III, meaning the actual scan $z$ matches the estimated scan, we can know that sensor $i$ secure and hence $i \notin I_a$. 
A worse case is considered in Case IV, where the sensor $i$ and LiDAR sensor $z$ are both under attack. In this case, we first check on LiDAR scan $z$ and estimate $\tilde{r}$ by Alg. \ref{alg:FT-LiDAR_Est} with the scan excluding $c_j$. If the modified LiDAR scan is secure, we should relative pose $\tilde{r}_i\leq \theta_h$ and $\tilde{\zeta}_z^s \leq \bar{\zeta}_z^s$. 

To help illustration, we provide an example on an autonomous system equipped with a IMU sensor, a GPS sensor and a LiDAR sensor. We denote the state estimation of IMU and GPS as $\hat{x}_{IMU}$ and $\hat{x}_{GPS}$ respectively. Let $E$ denotes the event that $\zeta_z^s \leq \bar{\zeta}^s$ and $r\leq \theta_h$. Let $\tilde{E}$ denotes the event that $\tilde{\zeta}_z^s \leq \bar{\zeta}_z^s$ and $r\leq \theta_h$. 
We can draw the conclusion on the attack pattern by the following table. 
\begin{table}[h]
    \centering
    \begin{tabular}{|c c c c|c|}
        \hline
        $E_{IMU}$ & $\tilde{E}_{IMU}$ & $E_{GPS}$ & $\tilde{E}_{GPS}$ & Conclusion \\
        \hline
        T & T & T & T & All Secure\\
        % T & T & - & - & IMU is Secure\\
        % - & - & T & T & IMU is Secure\\
        F & T & - & - & IMU is Secure\\
        - & - & F & T & GPS is Secure\\
        \hline
    \end{tabular}
    \caption{Example on FT-Estimator of an autonomous system equipped with IMU, GPS and LiDAR sensors}
    \label{tab:my_label}
\end{table}

For estimation $i$, let $\theta_l^i=\bar{\zeta}_i/2$.

\begin{theorem}
\label{th:ftest}
    Given convergent result $r_i=x-\hat{x}_i$ and $\bar{\zeta}_s$, for sensor $i\in I\backslash I_a$ given by criteria I-IV, we have estimation error exponentially bounded as $\|x-\hat{x}_i\|\leq \bar{\zeta}_i$ if Assumption \ref{assump:dtekf} holds. 
\end{theorem}
\begin{proof}
    We prove the claim by contradiction. Assume that there exist a sensor $b\in I\backslash I_a$, whose estimation $\hat{x}_b$ satisfies $\|x-\hat{x}_b\|\geq \bar{\zeta}_b$. 
    Sensor $b$ can be included into $I\backslash I_a$ by Case I, III and IV b).
    \begin{itemize}
        \item In Case I, we set $\theta_l=\min_i{\bar{\zeta}_i}/2$. 
        % For any sensor $i$, we can have estimation error $\zeta_i$ and threshold $\theta_l^i$. 
        If sensor $b$ has the estimation error $\|x-\hat{x}_b\|\geq \bar{\zeta}_b$, then we can have $\|x-\hat{x}_b\|\geq \theta_l$ by triangular inequality. Hence sensor $b$ will be excluded, which contradict to $b\in I\backslash I_a$. 
        % Then we can have sensor $b$ has the estimation error $\zeta_b$ sensor $b$ will not be included, which contradict to $b\in I\backslash I_a$. 
        \item In Case III, since $r$ is converge result and $\zeta_b^s \leq \bar{\zeta}^s$, we can know that LiDAR scan matches with estimated scan with relative pose change $r=x-\hat{x}_b$. There always exists a $\theta_h^b\leq\bar{\zeta}_b$ such that sensor $b$ will not be included, when $\|x-\hat{x}_b\|\geq \bar{\zeta}_b$. Hence, it contradicts to $b\in I\backslash I_a$. 
        \item In Case IV, we have original LiDAR scan spoofed $\zeta_z^s \geq \bar{\zeta}^s$ but filtered LiDAR scan matching the estimated scan $\tilde{\zeta}_z^s \leq \bar{\zeta}^s$. Similar to Case III, we can have $\tilde{r}=x-\hat{x}_b$. Then, there always exists a $\theta_h^b\leq\bar{\zeta}_b$ such that sensor $b$ will not be included, when $\|x-\hat{x}_b\|\geq \bar{\zeta}_b$. Hence, it contradicts to $b\in I\backslash I_a$.  
    \end{itemize}
    Otherwise, sensor $b$ will be excluded into set $I_a$ and hence for any sensor $i\in I\backslash I_a$ we can have the error bounded. 
    
    % For Case III and IV b), we consider the following two cases. If $r$ is converge result, there always exists a $\theta_h\in [\bar{\zeta}_i/2,\bar{\zeta}_i]$ to rise contradiction. \textcolor{blue}{If $r$ is not a converge result, the error bound \eqref{eq:scannoise} does not hold. Hence $b$ will not be excluded and contradiction rises. (Not sure about this)}
\end{proof}
\fi
% \textcolor{blue}{Next Step: FT-control and safety proof}

% \begin{itemize}
%     \item Case I: For any $i,j\in I_l$ ($i\neq j$), $\zeta_{i,j}\leq \theta_l$
%     \item Case II: If there exist a nonempty set of indices $Z\subsetneq I_l$ such that for any sensor indexing $i\in Z$ and $j\in I_l\backslash Z$, there exist $\zeta_{i,j}:=\|\hat{x}_i-\hat{x}_j\|> \theta_l$. 
%     % \begin{itemize}
%     %     \item a) For any sensor $i\in Z$  $\mathcal{O}_i(\hat{x}_{i}, \mathcal{M})\ominus \mathcal{O}(x,S)$
%     % \end{itemize}
%     \item Case III: For some estimation $\hat{x}_i, i\in Z$, we have $\Lambda_i:=\mathcal{O}_i(\hat{x}_{i}, \mathcal{M})\ominus \mathcal{O}(x,S)\geq \theta_h$ and $\tilde{\Lambda}_i:=\mathcal{O}_i(\hat{x}_{i}, \mathcal{M}\backslash c)\ominus \mathcal{O}(x,S\backslash c)< \theta_h$, where $c$ is the output of Alg. \ref{alg:FT-LiDAR_Est}. 
% \end{itemize}

 
% that determined likely to be spoofed by the FT-Estimator. 

% Theorem 2 $Z[k]=\{y(x[k]), \mathcal{O}(\Bar{\mathcal{I}})\}$

% We then select parameters for fault tolerance $\theta_l, \theta_h>0$ and $\delta>0$. We define the following cases to help illustration of the FT-scheme. 
% \begin{itemize}
%     \item Case I: For any $i,j\in I_l$ ($i\neq j$), $\zeta_{i,j}:=\|\hat{x}_i-\hat{x}_j\|\leq \theta_l$
%     \item Case II: If there exist a nonempty set of indices $Z\subsetneq I_l$ such that for any sensor indexing $i\in Z$ and $j\in I_l\backslash Z$, there exist $\zeta_{i,j}:=\|\hat{x}_i-\hat{x}_j\|> \theta_l$. 
%     % \begin{itemize}
%     %     \item a) For any sensor $i\in Z$  $\mathcal{O}_i(\hat{x}_{i}, \mathcal{M})\ominus \mathcal{O}(x,S)$
%     % \end{itemize}
%     \item Case III: For some estimation $\hat{x}_i, i\in Z$, we have $\Lambda_i:=\mathcal{O}_i(\hat{x}_{i}, \mathcal{M})\ominus \mathcal{O}(x,S)\geq \theta_h$ and $\tilde{\Lambda}_i:=\mathcal{O}_i(\hat{x}_{i}, \mathcal{M}\backslash c)\ominus \mathcal{O}(x,S\backslash c)< \theta_h$, where $c$ is the output of Alg. \ref{alg:FT-LiDAR_Est}. 
% \end{itemize}
% Case I is straight forward that we have all estimations are within a fault tolerance $\theta_l$. We do not need to exclude any sensor in this case. Case II and III can be tricky, since we do not know which sensor has the correct estimation and the adversary can spoof multiple sensor to overwhelm the traditional voting system. Hence, we need to use additional information to help exclude biased estimations. For estimation indexing $i$, we can refer the following criteria to determine whether we need to exclude it. 

% \textcolor{blue}{Table here for criteria}

% \textcolor{blue}{IMU, GPS LiDAR as an example}
% \begin{itemize}
%     \item If $\zeta_{i,j}\geq \theta_l$
% \end{itemize}

% As mentioned in the preliminaries, the error bound of state estimation of proprioceptive sensors with index $i$ using discrete-time EKF can be denoted as $\Bar{\zeta}_{i}$. 

% The set of feasible control inputs is defined at each time-step $k$ using the following steps:
% \begin{enumerate}
%     \item Define state estimation excluding sensor $i$ as $\hat{x}_{k,i}$ and control input $u_i:=\min\pi(\hat{x}_{i})$. Define a collection of a set $\Omega_{i\in I\backslash I_a}:= (u-u_i)^T (u-u_i) \leq \eta$, where $I_a=\emptyset$. 
%     If control input $u \in \bigcap_{i\in I\backslash I_a} \Omega_{i}$, set $\hat{u}=0$. Otherwise, select $u_{\alpha}[k]$ such that $u_o:=u+u_{\alpha}$ is the solution to the following QCQP problem. 
%     \begin{equation}
%     \begin{split}
%         \ &{\min\pi(\hat{x}_{i})}\\
%         s.t. \ & u_o \in \bigcap_{i\in I\backslash I_a} \Omega_{i}
%     \end{split}
%     \end{equation}
%     If no such $u_{t}$ exists, then go to Step 2. 
    
%     \item Exclude false measurement with criteria I-IV and update $I_a$
    
%     \item Remove the indices $i$ from $I$ corresponding to the estimators with the largest residue values $y_{k, i}-o_{i} (\hat{x}_{t, i})$ until there exists $u_{k} \in \bigcap_{i \in I\backslash I_a} \Omega_{i}$.
% \end{enumerate}

% \begin{enumerate}
%     \item Define state estimation excluding sensor $i$ as $\hat{x}_{k,i}$ and control input $u_i:=\pi(\hat{x}_{k,i})$. Define a collection of a set $\Omega_{i\in I\backslash I_a}:= (u-u_i)^T (u-u_i) \leq \eta$. 
%     % \begin{multline}
%     % \label{eq:safecons}
%     %     \Omega_i \triangleq \{ -\mathbb{E}[B(f(\hat{x}_{k,i})+g(\hat{x}_{k,i})u[k]) \mid \hat{x}_{k,i}]+ \\ \frac{B(\hat{x}_{k,i})}{\tilde{\alpha}} 
%     %     +\tilde{\beta} -\lambda_{\mathcal{X} \backslash \mathcal{X}_{u}}(x) s_{\mathcal{X} \backslash \mathcal{X}_{u}}(x) \in \Sigma[x]  \} 
%     % \end{multline}
%     If control input $u$ satisfies $u[k] \in \bigcap_{i\in I} \Omega_{i}$, set $u_{\alpha}[k]=0$. Otherwise, select $u_{\alpha}[k]$ such that $u_o:=u+u_{\alpha}$ is the solution to the following QCQP problem. 
%     \begin{equation}
%     \begin{split}
%         \min_{u_o} \ &{u_o^{T} R u_o+\hat{x}_i[k]^{T} P[k] B u_o+s[k]^{T} B u_o}\\
%         s.t. \ & u_o \in \bigcap_{i\in I\backslash I_a} \Omega_{i}
%     \end{split}
%     \end{equation}
%     If no such $u_{t}$ exists, then go to Step 2. 
    
%     \item For each $i$ with $ScanMatch(\mathcal{O}_i(\hat{x}_{k,i}, \mathcal{M}), \mathcal{O}(x_k,\Bar{\mathcal{I}}))>\theta_{h}$, we consider the following two cases: \\
%     \textbf{Case I: } If $i$ with $\left\|\hat{x}_{k, i}-\hat{x}_{k, I\backslash i}\right\|_{2}>\theta_{l}$, exclude sensor with index $i$ and set $\Omega_{k}=\Omega_{k} \backslash\{i\in I_l\}$. \\
%     \textbf{Case II: } Otherwise, exclude observation $\mathcal{O}$ and set $\Omega_{k}=\Omega_{k} \backslash\{i \in I_h\}$. \\
%     For the above cases, if $\bigcap_{i\in I} \Omega_{i} \neq \emptyset$, then select $u_{k} \in \bigcap_{i\in I} \Omega_{i}$. Else go to Step 3 .
    
%     % For each $i, j$ with $\left\|\hat{x}_{t, i}-\hat{x}_{t, j}\right\|_{2}>\theta_{i j}$, set $Z_{t}=Z_{t} \backslash\{i\}$ (resp. $Z_{t}=Z_{t} \backslash\{j\}$ ) if $\left\|\hat{x}_{t, i}-\hat{x}_{t, i, j}\right\|_{2}>\theta_{i j} / 2$ (resp. $\left.\left\|\hat{x}_{t, j}-\hat{x}_{t, i, j}\right\|_{2}>\theta_{i j} / 2\right)$. If $\bigcap_{i \in Z_{t}} \Omega_{i} \neq \emptyset$, then select $u_{t} \in \bigcap_{i \in Z_{t}} \Omega_{i}$. Else go to Step 3 .
    
%     \item Remove the indices $i$ from $Z_{t}$ corresponding to the estimators with the largest residue values $\bar{y}_{k, i}-\bar{h}_{i} (\hat{x}_{t, i})$ until there exists $u_{k} \in \bigcap_{i \in Z_{t}} \Omega_{i}$.
% \end{enumerate}

The set of feasible control inputs is defined at each time-step $k$ using Alg. \ref{alg:FTScheme}. 
\begin{algorithm}
\caption{Fault Tolerant Scheme}
\begin{algorithmic}
    \State We maintain $p$ EKFs for each sensor to estimate state $\hat{x}_i, \ i\in I := \{1,2,\ldots, p\}$.
    \State Initialize $I_a=\emptyset$
    \State Initialize $\Omega_{i\in I\backslash I_a}:= \{ u: (u-u_i)^T (u-u_i) \leq \eta$\}. 
    % \State Obtain estimate scan $\hat{O}_i(\hat{x}_i, \mathcal{M})$.
    \State Compute control input $u:=\min\pi(\hat{x}_{i},u)$. 
    \If{control input $u \in \bigcap_{i\in I\backslash I_a} \Omega_{i}$}
        \State set $\hat{u}=0$ and $u_o = u+\hat{u}$
    \Else
        \Comment{STEP 1} 
        \State Compute control input $\hat{u}$ such that $u_o:=u+\hat{u}$ is the solution to the following problem. 
        \begin{equation}
        \begin{split}
        \label{eq:qcqp}
            \ &{\min_{u_o}\pi(\hat{x}_{i},u_o)}\\
            s.t. \ & u_o \in \bigcap_{i\in I\backslash I_a} \Omega_{i}
        \end{split}
        \end{equation}
        \If{no such $u_o$ can be found}
        \Comment{STEP 2}
            \State Perform FT-LiDAR Estimation (Alg. \ref{alg:FT-LiDAR_Est}).
            \State Exclude false sensor with criteria I-IV into $I_a$.
            \State Compute $\hat{u}$ by solving \eqref{eq:qcqp}.
            \If{no such $u_o$ can be found}
                \Comment{STEP 3} 
                \For{$u\notin \bigcap_{i \in I\backslash I_a} \Omega_{i}$}
                    \State Compute residue values $y{i}-o (\hat{x}_{i})$
                    \State Include $i$ into $I_a$ with the largest residue. 
                \EndFor
            \EndIf
        \EndIf
    \EndIf
    
\end{algorithmic}
\label{alg:FTScheme}
\end{algorithm}

% Algorithm (transformation) = ML-NDT$(R,S,q,n,s)$

% \begin{algorithm}
% \caption{Fault Tolerant Control}
% \begin{algorithmic}
%     \State Given a safe region $\mathcal{C}$ and an accurate map $\mathcal{M}$
%     \State Given a verified safe trajectory $\mathcal{T}_s$. 
%     \For{$k\leq K$}
%         \State Fault Tolerant State Estimation $\hat{x}[k]$ with index $I[k]$.
%         \State Choose $u\in \Omega_{I[k]}$
%     \EndFor
% \end{algorithmic}
% \label{alg:FTCon}
% \end{algorithm}

% To ensure the system remain in safe region under adversarial attack, we consider the worst-case scenario when conducting safety verification.  
% The control module $u(\hat{x}[k], \mathcal{T})$ maps state estimation $\hat{x}[k]$ with a given trajectory $\mathcal{T}$ to control input $u[k]$ to maneuver the physical plant. 

% \subsection{Performance Trade-off}
% \begin{proposition}
% Verified safe trajectories $\mathcal{T}_s\in \Bar{\mathcal{T}}$ generated by planner who ensures convergence inherit the property of convergence.  
% \end{proposition}

% \subsection{Compatibility}
% We illustrate how our approach 
% To improve the compatibility to some path planning algorithms that focus more on performance, we propose a 

% term hd sensor and ld sensor
% low-dim sensors can be expressed as $y=\pi(x)$ but high-dim sensors need to be processed with filters feature extraction and etc. 

% this section is not novel
% focus more on perturbations


==> intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Timeline}
CBF Version: 
\begin{itemize}
    \item Theorem 2 Exponentially bounded: derive the error can be exponentially bounded under attack. The change can derive a tighter bound and can make the paper more coherent. (1 day)
    \item III. C change barrier certificate to control barrier function: given $\|x-\hat{x}\|$ (exponentially) bounded, construct a control policy to ensure safety. This part will replace section III. C and make proposition 1,2 a stronger contribution. (1 day)
    \item Simulation: make corresponding changes to the simulation case study II. (1 day)
    \item Intro and related work (2 days)
\end{itemize}

Barrier Certificate Version (current version): 
\begin{itemize}
    \item Revise section II (2 hours)
    \item Revise section III. D and E (3 hours)
    \item Simulation (1 day)
    \item Intro \& Related Work (2 days)
\end{itemize}



\subsection{Topic}
The sensors and perception are emphasized in \cite{goerzen2010survey} to play as much of a role as control and dynamics in UAV systems. Sensor measurements, as the input of simultaneous mapping and planning (SMAP) in a UAV system, can determine the quality and reliability of the system performance. Noisy data or false data injected by adversary may biased the state estimation and the output of SMAP resulting in false path planning and control policy, which may increases the risk of unsafe behaviors and may even causes collisions.  

\textbf{Motivation: }GPS-spoofing attack can cause collision and insecure behaviors due to inaccurate localization of GNSS, which is extremely dangerous for safety critical systems such as self-driving car, unmanned  vehicle (UV) including aerial and ground (UAV/UGV). Hence, it is important to design an approach to either diagonalize attacks or to achieve FTC. 

\textbf{Problem Statement: }Consider an Unmanned Vehicle (UV) system equipped with multiple sensors with low-dimensional data such as IMU, GPS, INS, etc as well as sensors with high-dimensional data like LiDAR and camera. Our goal is to ensure the system remains in a predefined region when it experiences sensor fault or spoofing attack.

Perturbations analysis in complex systems, such as neural network, can be challenging in soundness and computationally feasibility, which usually requires additional design in robustness (ReLU [Singh, Gagandeep, et al. 2018 NIPS]). Environmental observations, with high-dimensional data, are usually processed by a series of sensor fusion or neural networks, which makes it challenging to track the impact of perturbations.

\subsection{Potential Contributions}
\begin{itemize}
    \item We propose a discrete-time control barrier certificates with synthesis to deal with adversarial input perturbation. 
    \begin{itemize}
        \item Discrete-time CBC
        \item Synthesis to ensure safety under FDI
    \end{itemize}
    \item To fill the gap between theoretical and implementation contribution, we proposed a framework, compatible with LiDAR-based systems with only minor modifications, to ensure safety under perturbations. 
    \begin{itemize}
        \item Framework Structure
        \item \textcolor{blue}{NDT-based LiDAR FT-Estimation (By Tuesday)}
    \end{itemize}
    \item We specify the proposed method onto a LiDAR-based system, with a FT-estimator proposed to exclude false data and a computationally feasible approach to deal with the impact of input perturbations by projecting possible estimated states into observation space. 
    \begin{itemize}
        \item FT-estimator
        \item \textcolor{blue}{Algorithm of FT-Estimator without assuming redundancy of LiDAR sensor}
        \item \textcolor{blue}{Safety guarantee for system with LiDAR}
    \end{itemize}
    \item We evaluate our approach in a UAV delivery case study
    \begin{itemize}
        \item Baseline
        \item \textcolor{blue}{FT-estimator by 3/2}
        \item \textcolor{blue}{CBC synthesis}
        \item \textcolor{blue}{Experiments w/o Attack}
    \end{itemize}
\end{itemize}

% \begin{itemize}
%     \item CBF for High-dimensional data
%     \item Safety framework for Lidar-based system under FDI
%     \item Grind on UAV platform
%     \item Evaluate by simulating a UAV case study.
% \end{itemize}



==> prelim.tex <==
\section{Preliminary Background}\label{sec:preliminary}

\subsection{LiDAR}

\subsection{Path Planning}

\subsection{Barrier Certificate}

\begin{lemma}
    Proposition 2. Given (2) and the sets $\mathcal{X} \subset \mathbb{R}^{n}, \mathcal{X}_{u} \subseteq \mathcal{X}, \mathcal{X}_{0} \subseteq$ $\mathcal{X} \backslash \mathcal{X}_{u}$ with $F(x, \xi)=f(x)+g(x) u(x)+\sigma(x) \xi$ where $u(x)$ is some feedback control law. Suppose there exists a function B such that
    \begin{eqnarray}
        B(x) &\leq& \gamma \ \forall x \in \mathcal{X}_{0}, \\
        B(x) &\geq& 1 \ \forall x \in \mathcal{X}_{u}, \\
        B(x) &\geq& 0 \ \forall x \in \mathcal{X}, \text { and } \\
        \mathbb{E}[B(F(x, \xi)) \mid x] &\leq& \frac{B(x)}{\tilde{\alpha}}+\tilde{\beta} \quad \forall x \in \mathcal{X} \backslash \mathcal{X}_{u}
    \end{eqnarray}
    for some $\tilde{\alpha} \geq 1,0 \leq \tilde{\beta}<1$ and $\gamma \in[0,1)$. Define 
    \begin{eqnarray}
        \rho_{u}&:=&P\left\{\tilde{x}[k] \in \mathcal{X}_{u} \text { for some } 0 \leq k \leq N \mid \tilde{x}[0] \in \mathcal{X}_{0}\right\} \\
        \rho_{B}&:=&P\left\{\sup _{0 \leq k \leq N} B(\tilde{x}[k]) \geq 1 \mid \tilde{x}[0] \in \mathcal{X}_{0}\right\}
    \end{eqnarray}
    where $\tilde{x}[k]$ is a stopped solution of (2). Then
    \begin{itemize}
        \item If $\tilde{\alpha}>1$ and $\frac{\tilde{\beta} \tilde{\alpha}}{\tilde{\alpha}-1} \leq 1$,
        $$
        \rho_{u} \leq \rho_{B} \leq 1-(1-\gamma) \prod_{0}^{N-1}(1-\tilde{\beta})
        $$
        \item If $\tilde{\alpha}>1$ and $\frac{\tilde{\beta} \tilde{\alpha}}{\tilde{\alpha}-1}>1$,
        $$
        \rho_{u} \leq \rho_{B} \leq \gamma \tilde{\alpha}^{-N}+\frac{\left(1-\tilde{\alpha}^{-N}\right) \tilde{\alpha} \tilde{\beta}}{(\tilde{\alpha}-1)}
        $$
        \item If $\tilde{\alpha}=1$,
        $$
        \rho_{u} \leq \rho_{B} \leq \gamma+\tilde{\beta} N .
        $$
    \end{itemize}
\end{lemma}


==> simulation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case Study}\label{sec:simulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section evaluates our proposed approach on a UAV delivery system in an urban environment.
% A simulation of our approach on a UAV delivery system is described as follows. 
%We first describe the case study settings. Then we compare our proposed approach with a baseline approach. 
% The first case study evaluates the fault-tolerant estimation approach of Section \ref{sec:ft-LiDAR est} and \ref{sec:ft-state est}. The second case study evaluates our end-to-end safe control framework.
% \subsection{Simulation Setting}
The UAV system is based on MATLAB UAV Package Delivery Example \cite{UAVDelivery}. 
% The system is state-feedback maneuvered by PID controllers for stability, velocity and altitude. We denote the state at time step $k$ as
% $x[k]=[[x]_1,[x]_2]^\top_k$, where $[x]_1$ and $[x]_2$ represent the position of UAV on $X$-axis and $Y$-axis, respectively. 
% Our goal is to control the position of the UAV system with dynamic model identified by MATLAB system identification toolbox as:  
We denote the state at time step $k$ as $x[k]=[[x]_1,[x]_2]^\top_k$, where $[x]_1$ and $[x]_2$ represent the position of UAV on $X$-axis and $Y$-axis, respectively. 
Our goal is to control the position of the UAV system. 
The system is state-feedback maneuvered by PID controllers for stability, velocity and altitude with dynamic model identified by MATLAB system identification toolbox as:  
\begin{multline}
    \label{eq:uav_dyna}
    \begin{bmatrix}
    [x]_1\\
    [x]_2
    \end{bmatrix}_{k+1}
    =
    \begin{bmatrix}
    1 & -4.29\times 10^{-5}\\
    -1.47\times 10^{-5} & 1
    \end{bmatrix}
    \begin{bmatrix}
    [x]_1\\
    [x]_2
    \end{bmatrix}_{k}\\
    +
    \begin{bmatrix}
    0.0019 & -1.93\times 10^{-5}\\
    -2.91\times 10^{-4} & 0.0028
    \end{bmatrix}
    \begin{bmatrix}
    [u]_1\\
    [u]_2
    \end{bmatrix}_{k}.
\end{multline}
The UAV has one LiDAR sensor and two inertial navigation system (INS) sensors, namely, INS1 and INS2. The UAV maintains two EKFs associated with each INS sensor to estimate its position at each time $k$, denoted as $\hat{x}_1[k]$ and $\hat{x}_2[k]$, respectively. 

There exists a malicious adversary who can compromise one of the INS sensors and spoof the LiDAR sensor \cite{cao2019adversarial}. 
% The adversary has the capacity choose any one of the INS sensors to compromise and is capable of spoofing the LiDAR sensor within an angle of $10^{\circ}$.
% We set the thresholds $\theta_h$ and $\bar{\zeta}_s$ as $\theta_h=2$ and $\bar{\zeta}_s=375$, respectively. 
We compare our proposed approach with a baseline utilizing a PID controller with state estimation given by INS1.

% For comparison, we set the baseline controller to be a PID controller taking estimation from INS1. 
% \subsection{Case Study I: Fault Tolerant Estimation}
% A numerical study of the proposed FT-Estimation for LiDAR-based system was performed using Matlab. The goal of the FT-Estimation is to identify conflict sensor under false data injection (FDI) attack and LiDAR spoofing attack. 

% In the first scenario, the adversary attacks one INS sensor to bias the UAV along x-axis by $-20$ meters. To identify which INS sensor is under attack, the FT-Estimation algorithm is used. The comparison between the LiDAR scan and the point cloud data estimated based on position information from INS sensor is shown in Fig. 1. 
% We evaluate the performance under FDI attack on INS sensor and joint FDI attack and LiDAR spoofing attack. 
We first evaluate the performance of our proposed fault-tolerant estimation under FDI attack. The adversary biases INS1 sensor by $-20$ meters on $X$-axis. 

% The results are shown in Fig . We scatter the actual position with green diamond and plot the estimated actual LiDAR observations.  
In Fig. \ref{fig:s1x1}, a significant drift can be observed between estimated LiDAR observation $\mathcal{O}(\hat{x}_1,\mathcal{M})$ and actual LiDAR observation $\mathcal{O}(x,S)$. In Fig. \ref{fig:s1x2}, the estimated LiDAR observation $\mathcal{O}(\hat{x}_2,\mathcal{M})$ aligns with the actual LiDAR observation. FT-Estimation outputs $2$ indicating INS1 is not trusted and INS2 is trusted. 

We next evaluate the performance under both FDI attack on INS sensor and LiDAR spoofing attack. The adversary biases INS1 sensor by $-20$ meters on $X$-axis and generates a random obstacle within range of $[10,15]$ meters and angle of $[-70,-60]$ degrees. 
In Fig. \ref{fig:s2x1}, a significant drift can be observed between estimated LiDAR observation $\mathcal{O}(\hat{x}_1,\mathcal{M})$ and actual LiDAR observation $\mathcal{O}(x,S)$. Besides, actual LiDAR observation has an obstacle at position $(5.5, -11.6)$ generated by the LiDAR spoofing attack. In Fig. \ref{fig:s1x2}, the obstacle points generated by the LiDAR spoofing attack are eliminated by FT-Estimation algorithm and the estimated LiDAR observation $\mathcal{O}(\hat{x}_2,\mathcal{M}\backslash c)$ aligns with the reconstructed LiDAR observation $\mathcal{O}(x,S\backslash c)$. FT-Estimation outputs $2$ indicating INS1 raises conflict and INS2 is trusted.  
%%%%%%%%%
%In Fig. 1(c), a significant drift can be observed between estimated LiDAR observation $\mathcal{O}(\hat{x}_1,\mathcal{M})$ and actual LiDAR observation $\mathcal{O}(x,S)$. Besides, actual LiDAR observation has an obstacle at [] generated by the LiDAR spoofing attack. In Fig. 1(d), the obstacle points generated by the LiDAR spoofing attack are eliminated by FT-Estimation algorithm, two LiDAR observations align. FT-Estimation outputs $2$ indicating INS1 raises conflict and INS2 is trusted.  
%%%%%%%%%
% The results are shown in Fig . We scatter the actual position with green diamond and plot the estimated actual LiDAR observations. 

\begin{figure*}[]
\centering
\begin{subfigure}{.25\textwidth}
% \title{Training Episodes}
  \centering
  \includegraphics[width = \textwidth]{Figs/cs1_1ins1L.eps}
  \subcaption{}
  \label{fig:s1x1}
\end{subfigure}%
\hfill
\begin{subfigure}{.25\textwidth}
% \title{Testing Episodes}
  \centering
  \includegraphics[width = \textwidth]{Figs/cs1_1ins2L.eps}
  \subcaption{}
  \label{fig:s1x2}
\end{subfigure}%
\hfill
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/cs1_2ins1sLs.eps}
%   \caption{Joint FDI and Spoofing Attack: INS1 estimation}
  \subcaption{}
  \label{fig:s2x1}
\end{subfigure}%
\hfill
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figs/cs1_2ins2Lc.eps}
%   \caption{Joint FDI and Spoofing Attack: INS2 estimation}
  \subcaption{}
  \label{fig:s2x2}
\end{subfigure}%
\caption{Numerical Study 1 FT-Estimation Result: (a) and (b) are estimated and actual LiDAR observation comparisons. (c) and (d) are estimated and reconstructed LiDAR observation}
\end{figure*}

% Fig.1: When one INS sensor is under attack, FT estimation algorithm is used to evaluate which INS sensor works without attack through comparing LiDAR scan and estimated point cloud based on the position information from INS. (a) When the INS1 is under attack, the estimated point cloud will significantly drift compared with that of the LiDAR. (b) When INS2 is not under attack, the point cloud estimated based on its position information will match with that of the LiDAR with a tiny drift.
% As shown in Fig.2, when using FT Estimation, only based on the position information provided by INS2 can the obstacle of LiDAR be eliminated.  Therefore, the difference score between self-matching estimated point cloud and matching between estimated point cloud and LiDAR scan is under score threshold and the position difference is under position threshold. 

\subsection{Case Study II: Fault Tolerant Control}
We evaluate the performance of our fault-tolerant control framework under FDI attack.
We set the threshold for scan match as $\theta_h=2$ and the threshold for scan match score as $\bar{\zeta}_s=375$. We formulate a half-plane unsafe area described as $x_2>-100$. 
In order to test the safety, an adversary is present to bias INS1 sensor by $-20$ meters when $[x]_2\leq 55$ meters. 

% %%%%%%%%%%%%
% For baseline, when y<=55, the UAV gets attack. Getting attack time is from 37.255 s, and it will enter into unsafe area at 46.955 s.
% For proposed method, when y<=55, the UAV gets attack. Getting attack time is from 101.2750 s, and it will not enter into unsafe area.
% %%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width = 0.38\textwidth]{Figs/cs2_traj2.eps}
    \caption{Numerical Study 2: FT-Framework Result: Comparison of trajectories of UAV system controlled by baseline and proposed FT-Framework}
    \label{fig:cs2_ftframe}
\end{figure}

% For baseline, the UAV system is under FDI attack since $37.255s$. 
As shown in Fig. \ref{fig:cs2_ftframe}, the UAV system under FDI attack with baseline controller reaches the unsafe area, while the one with proposed framework remains in the safe region. 

% \begin{equation}
%     \label{eq:uav_dyna}
%     .
% \end{equation}
% With a PID velocity controller in a velocity control loop, we can further formulate the feedback system as 
% \begin{equation}
%     \label{eq:uav_fbdyna}
%     .
% \end{equation}
% We consider the UAV system equipped with a IMU sensor and a GPS sensor to detect global position $x_x, x_y$ and orientation $x_\phi$

% and a 2-D LiDAR sensor. 
% \begin{equation}
%     \label{eq:uav_obs}
%     .
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%         x_{k+1} = &A x_k + B u(\hat{x}_{\alpha}[k]) + B \hat{u}[k]  + w[k]\xi[k] \\
%         \hat{x}_{k+1} =& A \hat{x}_k + B u(\hat{x}_{\alpha}[k])  + K_k(o(x[k]) + v[k]\eta[k] - o(\hat{x}[k])) \\
%         K_k =& A_{k} P_{k} C_{k}^{T}(C_{k} P_{k} C_{k}^{T}+R_{k})^{-1} \\
%         P_{k+1} =& A_{k} P_{k} A_{k}^{T}+Q_{k}-K_{k}(C_{k} P_{k} C_{k}^{T}+R_{k}) K_{k}^{T}.
%     \end{aligned}
% \end{equation}

% \begin{multline}
% \label{eq:extend_dyn}
%     \Bar{x}[k+1] = A \Bar{x}[k] + B (u(\bar{B} \bar{x}_{\alpha})+\hat{u}[k]) + \\ \bar{W}_{k} w[k]\xi[k] + \bar{V}_{k} v[k]\eta[k], 
% \end{multline}
% where 
% \begin{equation}
%     \bar{B}_{k}=\left(\begin{array}{c}0 \\ I\end{array}\right), \quad
%     \bar{W}_{k}=\left(\begin{array}{c}I \\ 0\end{array}\right), \quad \bar{V}_{k}=\left(\begin{array}{c}0 \\ K_k\end{array}\right). 
% \end{equation}
% where $u(\bar{B} \bar{x}_{\alpha})$

% where $x_1$ is the rotor current, $x_2$ is the angular velocity, $u\in\mathcal{U}=[-1,1]$ is the stator current. The parameters in the system dynamics are unknown, and are normally obtained empirically in practice. 




